Thompson Sampling with Approximate Inference

We study the effects of approximate inference on the performance of Thompson sampling in the $k$-armed bandit problems. Thompson sampling is a successful algorithm for online decision-making but requires posterior inference, which often must be approximated in practice. We show that even small constant inference error (in $\alpha$-divergence) can lead to poor performance (linear regret) due to under-exploration (for $\alpha<1$) or over-exploration (for $\alpha>0$) by the approximation. While for $\alpha > 0$ this is unavoidable, for $\alpha \leq 0$ the regret can be improved by adding a small amount of forced exploration even when the inference error is a large constant.

==> diagram.tex <==
\begin{figure*}
	\centering
 \begin{subfigure}[b]{0.07\textwidth}
 	\begin{tikzpicture}
 	[align=center,node distance=1cm]
 	\node (pi0) [dist] {$\Pi_0$};
 	\node (A1) [action, right of = pi0] {$A_1$};
 	\node (pi1) [dist, below of= pi0] {$\Pi_1$};
 	\node (A2) [action, right of = pi1] {$A_2$};
 	\node (pi2) [dist, below of =pi1] {$\Pi_2$};
 	\node (A3) [action, right of = pi2] {$A_3$};
 	\draw [thick, ->] (pi0) -- (A1);
 	\draw [thick, ->] (pi1) -- (A2);
 	\draw [thick, ->]  (pi2) -- (A3);
 	\draw [thick, ->]  (pi0) -- (pi1);
 	\draw [thick, ->]  (pi1) -- (pi2);
 	\draw [thick, ->]  (A1) -- (pi1);
 	\draw [thick, ->] (A2) -- (pi2);
 	\end{tikzpicture}
 	\end{subfigure}
 	\hfill
 	\begin{subfigure}[b]{0.1\textwidth}
 		\begin{tikzpicture}
 		[align=center,node distance=1cm]
 		\node (pi0) [dist] {$\Pi_0$};
 		\node (q0) [approx_dist, right of = pi0] {$Q_0$};
 		\node (A1) [action, right of = q0] {$A_1$};
 		\node (pi1) [dist, below of= pi0] {$\Pi_1$};
 		\node (q1) [approx_dist, right of = pi1] {$Q_1$};
 		\node (A2) [action, right of = q1] {$A_2$};
 		\node (pi2) [dist, below of =pi1] {$\Pi_2$};
 		\node (q2) [approx_dist, right of = pi2] {$Q_2$};
 		\node (A3) [action, right of = q2] {$A_3$};
 		\draw [thick, ->] (pi0) -- (q0);
 		\draw [thick, ->] (pi1) -- (q1);
 		\draw [thick, ->]  (pi2) -- (q2);
 		 		\draw [thick, ->] (q0) -- (A1);
 		 		\draw [thick, ->] (q1) -- (A2);
 		 		\draw [thick, ->]  (q2) -- (A3);
 		
 		\draw [thick, ->]  (pi0) -- (pi1);
 		\draw [thick, ->]  (pi1) -- (pi2);
 		\draw [thick, ->]  (A1) -- (pi1);
 		\draw [thick, ->] (A2) -- (pi2);
 		\end{tikzpicture}
 	\end{subfigure}
 		\hfill
 		\begin{subfigure}[b]{0.2\textwidth}
 			\begin{tikzpicture}
 			[align=center,node distance=1cm]
 		
 				\node (pi0) [dist] {$\Pi_0$};
 				\node (q0) [approx_dist, right of = pi0] {$Q_0$};
 				\node (A1) [action, right of = q0] {$A_1$};
 				\node (pi1) [dist, below of= pi0] {$\Pi_1$};
 				\node (q1) [approx_dist, right of = pi1] {$Q_1$};
 				\node (A2) [action, right of = q1] {$A_2$};
 				\node (pi2) [dist, below of =pi1] {$\Pi_2$};
 				\node (q2) [approx_dist, right of = pi2] {$Q_2$};
 				\node (A3) [action, right of = q2] {$A_3$};
 				\draw [thick, ->] (pi0) -- (q0);
 				\draw [thick, ->] (pi1) -- (q1);
 				\draw [thick, ->]  (pi2) -- (q2);
 				\draw [thick, ->] (q0) -- (A1);
 				\draw [thick, ->] (q1) -- (A2);
 				\draw [thick, ->]  (q2) -- (A3);
 				
 				\draw [thick, ->]  (pi0) -- (pi1);
 				\draw [thick, ->]  (pi1) -- (pi2);
 		
 			\node (Aprime1) [action,left of = pi0] {$A'_1$};
 			\node (Aprime2) [action, left  of = pi1] {$A'_2$};
 			\node (Aprime3) [action, left  of = pi2] {$A'_3$};
 			\draw [thick, ->] (pi0) -- (Aprime1);
 			\draw [thick, ->] (pi1) -- (Aprime2);
 			\draw [thick, ->]  (pi2) -- (Aprime3);
 			\draw [thick, ->]  (Aprime1) -- (pi1);
 			\draw [thick, ->] (Aprime2) -- (pi2);
 			\end{tikzpicture}
 		\end{subfigure}
 		\hfill
 		\begin{subfigure}[b]{0.1\textwidth}
 			\begin{tikzpicture}
 			[align=center,node distance=1cm]
 			\node (pi0) [dist] {$\Pi_0$};
 			\node (q0) [approx_dist, right of = pi0] {$Z_0$};
 			\node (A1) [action, right of = q0] {$A_1$};
 			\node (pi1) [dist, below of= pi0] {$\Pi_1$};
 			\node (q1) [approx_dist, right of = pi1] {$Z_1$};
 			\node (A2) [action, right of = q1] {$A_2$};
 			\node (pi2) [dist, below of =pi1] {$\Pi_2$};
 			\node (q2) [approx_dist, right of = pi2] {$Z_2$};
 			\node (A3) [action, right of = q2] {$A_3$};
 			\draw [thick, ->] (pi0) -- (q0);
 			\draw [thick, ->] (pi1) -- (q1);
 			\draw [thick, ->]  (pi2) -- (q2);
 			\draw [thick, ->] (q0) -- (A1);
 			\draw [thick, ->] (q1) -- (A2);
 			\draw [thick, ->]  (q2) -- (A3);
 			
 			\draw [thick, ->]  (pi0) -- (pi1);
 			\draw [thick, ->]  (pi1) -- (pi2);
 			\draw [thick, ->]  (A1) -- (pi1);
 			\draw [thick, ->] (A2) -- (pi2);
 			\end{tikzpicture}
 		\end{subfigure}
 		\hfill
 		\begin{subfigure}[b]{0.2\textwidth}
 			\begin{tikzpicture}
 			[align=center,node distance=1cm]
 			
 			\node (pi0) [dist] {$\Pi_0$};
 			\node (q0) [approx_dist, right of = pi0] {$Z_0$};
 			\node (A1) [action, right of = q0] {$A_1$};
 			\node (pi1) [dist, below of= pi0] {$\Pi_1$};
 			\node (q1) [approx_dist, right of = pi1] {$Z_1$};
 			\node (A2) [action, right of = q1] {$A_2$};
 			\node (pi2) [dist, below of =pi1] {$\Pi_2$};
 			\node (q2) [approx_dist, right of = pi2] {$Z_2$};
 			\node (A3) [action, right of = q2] {$A_3$};
 			\draw [thick, ->] (pi0) -- (q0);
 			\draw [thick, ->] (pi1) -- (q1);
 			\draw [thick, ->]  (pi2) -- (q2);
 			\draw [thick, ->] (q0) -- (A1);
 			\draw [thick, ->] (q1) -- (A2);
 			\draw [thick, ->]  (q2) -- (A3);
 			
 			\draw [thick, ->]  (pi0) -- (pi1);
 			\draw [thick, ->]  (pi1) -- (pi2);
 			
 			\node (Aprime1) [action,left of = pi0] {$A'_1$};
 			\node (Aprime2) [action, left  of = pi1] {$A'_2$};
 			\node (Aprime3) [action, left  of = pi2] {$A'_3$};
 			\draw [thick, ->] (pi0) -- (Aprime1);
 			\draw [thick, ->] (pi1) -- (Aprime2);
 			\draw [thick, ->]  (pi2) -- (Aprime3);
 			\draw [thick, ->]  (Aprime1) -- (pi1);
 			\draw [thick, ->] (Aprime2) -- (pi2);
 			\end{tikzpicture}
 		\end{subfigure}
 			\caption{\label{fig:motivating_example_simulation_scheme} Simulation schemes}
\end{figure*}


==> proof_convert_distribution.tex <==
	\section{Proof of Lemma~\ref{lem:convert_distribution}}
	\label{sec:proof_convert_distribution}

	
%	Even though we consider the error when sampling the parameter $m$, the regret comes from choosing the wrong arm. In this section we relate the error when sampling the parameter $m$ to the error when sampling the arm $i$. 
%	
%	Let $\Pi_{t,i}$ denote $\Pi_t(\Omega_i)$ and $Q_{t,i}$ denote $Q_t(\Omega_i)$. Let $\overline{\Pi_t}$ denote the posterior distribution of the best arm with the density function
%	\begin{align}
%	\overline{\pi_t}(i) = P(A^* = i|H_{t-1}) = \int_{\Omega_i} \pi_t(m) dm = \Pi_{t,i} 
%	\end{align} 
%	
%	Let $\overline{Q_t}$ denote the approximation of $\overline{\Pi_t}$ with the density function
%	\begin{align}
%	\overline{q_t}(i)  = P(A_t = i|H_{t-1})= \int_{\Omega_i} q_t(m) dm = Q_{t,i}
%	\end{align} 
%	Because the $\alpha$-divergence is convex, we can apply Jensen's inequality to show that the $\alpha$-divergence between $\overline{\Pi_t}$  and $\overline{Q_t}$ is upper bounded by the $\alpha$-divergence between $\Pi_t$ and $Q_t$. 
%	\begin{lemma}
%		\label{lem:convert_distribution}
%		We have that
%		\begin{align}
%		D_{\alpha} (\overline{\Pi_t}, \overline{Q_t})  \leq D_{\alpha} (\Pi_t, Q_t)  
%		\end{align}
%	\end{lemma}

		
To convert between $D_{\alpha}(\Pi_t, Q_t)$ and $D_{\alpha}(\overline{\Pi_t } , \overline{Q_t})$ we first prove the following lemma:
	\begin{lemma}[Jensen's Inequality]
		\label{lem:Jensen}
		Let $f: \mathcal{R}^2 \rightarrow \mathcal{R}$ be a convex function. Let $P: \mathcal{R}^k \rightarrow \mathcal{R}$ and $Q: \mathcal{R}^k \rightarrow \mathcal{R}$ be 2 functions. Let $S$ is a subset of  $R^k$, the domain of $x$ and $|S|$ denote the volume of $S$. Then
		\begin{align}
		\label{eq:Jensen}
		&\frac{1}{|S|} \int_S  f(P(x),Q(x)) dx  \\&\geq f \left (  \frac{1}{|S|} \int_S P(x) dx , \frac{1}{|S|} \int_S Q(x) dx \right ) 
		\end{align}
	\end{lemma}
	\begin{proof}
		Multivariate Jensen's Inequality states that if $X$ is a n-dimensional vector random variable and $f: \mathcal{R}^n \rightarrow \mathcal{R}$ is a convex function then 
		\begin{align}
		 \mathbb{E}(f(X)) \geq f(\mathbb{E}(X)).
		\end{align}
		To use the multivariate Jensen's Inequality we define the $2$-dimensional vector random variable $X: S \rightarrow \mathcal{R}^2$ by 
		\begin{align}
		X(x)  := (P(x), Q(x)), 
		\end{align}
		and a probability distribution over $S$ such that for all $x \in S$: 
		\begin{align}
		\mathbb{P}(x) = \frac{1}{|S|}. 
		\end{align}
		Then the left-hand side of Eq.~\ref{eq:Jensen} becomes $\mathbb{E}(f(X))$, while the right-hand side becomes $ f(\mathbb{E}(X))$, and Eq. \ref{eq:Jensen} follows from the multivariate Jensen's Inequality. 
		\end{proof}

	Now we will prove Lemma~\ref{lem:convert_distribution}
	\begin{proof}[Proof of Lemma~\ref{lem:convert_distribution}]
		Since $D_{\alpha}(p,q)$ is convex \cite{Cichocki2010FamiliesOA}, the following function:
%	\begin{align}
%	\label{eq:alpha_divergence_0}
%	f(p, q) = q\log\frac{q}{p}
%	\end{align}
%	and 
	\begin{align}
	\label{eq:alpha_divergence_neq_0}
	f(p, q) = \frac{p^{\alpha}q^{1-\alpha}} {\alpha ( \alpha-1)}
	\end{align}
	is convex, and we can apply Lemma~\ref{lem:Jensen}: 
%	\begin{itemize}
		%\item When $\alpha = 0$:
%		\begin{align}
%		&D_{\alpha}(\Pi_t,Q_t) \\
%		=& \int q_t(m) \log \frac{q_t(m)}{\pi_t(m)} dm \\
%		=& \sum_{i} \int_{\Omega_i} q_t(m) \log \frac{q_t(m)}{\pi_t(m)} dm \\
%		\geq& \sum_{i} |\Omega_i| \frac{1}{|\Omega_i|} \int_{\Omega_i} q_t(m) dm \log \frac{\frac{1}{|\Omega_i|}\int_{\Omega_i} q_t(m) dm}{\frac{1}{|\Omega_i|}\int_{\Omega_i} \pi_t(m) dm}  \\
%		&\text{ by applying Lemma~\ref{lem:Jensen}} \\
%		=&  \sum_{i}  Q_{t,i} \log \frac{Q_{t,i}}{\Pi_{t,i}}   \\
%		=& D_{\alpha} (\overline{\Pi_t}, \overline{Q_t})
%		\end{align}
%		\item When $\alpha < 0$: 
		\begin{align}
		&D_{\alpha}(\Pi_t,Q_t) \\
		=&  \int \frac{\pi(x)^{\alpha}q(x)^{1-\alpha} - 1 }{-\alpha(1-\alpha)} dx\\
		=& \frac{-1}{\alpha(\alpha -1) } +  \sum_{i} \int_{\Omega_i} \frac{\pi(x)^{\alpha}q(x)^{1-\alpha} }{\alpha(\alpha-1)} dx  \\
		\geq& \frac{-1}{\alpha(\alpha -1) }  + \sum_{i}  |\Omega_i| \frac{ (\frac{\Pi_{t,i}}{|\Omega_i|})^{\alpha} (\frac{Q_{t,i}}{|\Omega_i|})^{1-\alpha}} {\alpha(\alpha-1)} \\
		&\text{ by applying Lemma~\ref{lem:Jensen}} \\
		=& \frac{-1}{\alpha(\alpha -1) }  + \sum_{i} \frac{\Pi_{t,i}^{\alpha} Q_{t,i}^{1-\alpha} } {\alpha(\alpha-1)}  \\
		=& D_{\alpha} (\overline{\Pi_t}, \overline{Q_t})
		\end{align}
	%	\end{itemize}
	\end{proof}
	

==> proof_thm_alpha_larger_than_0.tex <==
\section{Proof of Theorem \ref{thm:alpha_larger_than_0}}
\label{sec:proof_alpha_larger_than_0}
Let $\Omega_i \subseteq \Omega$ denote the region where arm $i$ is the best arm. Let $\Pi_{t,i}$ denote $\Pi_t(\Omega_i)$, the posterior probability that arm $i$ is the best arm. For $r > 1$, We construct the pdf of $Q_t$'s as follows: 
\begin{align}
\label{eq:Q_t_construction_alpha_larger_than_0}
 \frac{\pi_t(m)}{q_t(m)} = 
\begin{cases}
r,  &\text{if } m_1 > m_2 \\
\frac{1 - \Pi_{t,1}}{1 - \Pi_{t,1}/r}, &\text{ otherwise.}
\end{cases}
\end{align}
We will prove the theorem by the following steps:
\begin{itemize}
    \item In Lemma~\ref{lem:valid_distribution_alpha_larger_than_0} we show that $Q_t$'s are valid distributions. 
    \item In Lemma~\ref{lem:small_divergence1} we show that when $\alpha > 0$ the $\alpha$-divergence between $Q_t$ and $\Pi_t$ can be arbitrarily small 
    \item In Lemma~\ref{lem:regret1} we show that sampling from $Q_t$ for $\Theta(T)$ time-steps will generate linear regret, and lower bound the regret. 
\end{itemize}

\begin{lemma}
\label{lem:valid_distribution_alpha_larger_than_0}
If $\int \pi_t(m) dm = 1$ then the density function $q_t$ defined in Eq.~\ref{eq:Q_t_construction_alpha_larger_than_0} satisfies:
\begin{align}
\int q_t(m) dm = 1. 
\end{align}
\end{lemma}


\begin{lemma}
\label{lem:small_divergence1}
When $\alpha >0$, for all $\epsilon > 0$, for all $\Pi_t$, 
there exists $r >1$  such that  when $Q_t$'s are constructed from $r$ as shown in  Eq.~\ref{eq:Q_t_construction_alpha_larger_than_0}, $D(\Pi_t, Q_t) < \epsilon$

\end{lemma}
\begin{lemma}
\label{lem:regret1}
The expected regret of the policy that constructs $Q_t$'s as in Eq.~\ref{eq:Q_t_construction_alpha_larger_than_0} and sample from $Q_t$ for $T' =\theta(T)$ time-steps is linear and the lower bound of the average regret per time-step is
   \begin{align}
    L =
    \begin{cases}
    c\Delta(1- (1-\epsilon \alpha(1-\alpha))^{\frac{1}{1-\alpha}}), &\text{ if } \alpha > 1 \\
    c\Delta(1 - \frac{1}{e^{\epsilon}}), & \text{ if } \alpha = 1 \\
     c\Delta(1- (1-\epsilon  \alpha(1-\alpha))^{\frac{1}{1-\alpha}}),    & \parbox[t]{.3\columnwidth}{ if $0< \alpha < 1$ \\ and \\ $0 \leq \epsilon \leq \frac{1}{\alpha(1-\alpha)}$}. 
     \end{cases}, 
\end{align}
where $c = \frac{T'}{T}$ is $\Theta(1)$
\end{lemma}
%We plot the lower bound of the average regret per time step when $\Delta = 0.1$ as a function of $\epsilon$ in Fig~\ref{fig:regret_epsilon1}. 
%\begin{figure}[ht]
%	\centering
%	\includegraphics[width=\columnwidth]{fig/regret_epsilon1.png}
%	\caption{\label{fig:regret_epsilon1} Lower bound of regret per time step as a function of $\epsilon$ when $m_1 - m_2 = 0.1$ in the example in Theorem~\ref{thm:alpha_larger_than_0}}
%\end{figure}
\subsection{Proof of Lemma~\ref{lem:valid_distribution_alpha_larger_than_0}}
\begin{proof}
Assume that $\int \pi_t(m) dm = 1$, we will show that $\int q_t(m) dm = 1$: 
\begin{align}
  &\int q_t(m) dm \\ 
  &= \int_{\Omega_1}  q_t(m) dm + \int_{\Omega_2}  q_t(m) dm \\ 
  &= \int_{\Omega_1} \frac{1}{r} \pi_t(m) dm + \int_{\Omega_2}   \frac{1 - \Pi_{t,1}/r}{1 - \Pi_{t,1}} \pi_t(m) dm \\
  &= \frac{1}{r} \Pi_{t,1} + \frac{1 - \Pi_{t,1}/r}{1 - \Pi_{t,1}} \Pi_{t,2} \\
  &= \frac{1}{r} \Pi_{t,1} + \frac{1 - \Pi_{t,1}/r}{1 - \Pi_{t,1}} (1-\Pi_{t,1}) \\
  &= 1
\end{align}
\end{proof}
\subsection{Proof of Lemma~\ref{lem:small_divergence1}}
\begin{proof}
First we calculate the $\alpha$-divergence between $\Pi_t$ and $Q_t$ constructed in Eq.~\ref{eq:Q_t_construction_alpha_larger_than_0}. Let $\Omega_1 \subseteq \Omega$ denote the region where $m_1 > m_2$ and $\Omega_2 \subseteq \Omega$ denote the region where $m_2 \geq m_1$.

When $\alpha > 0, \alpha \neq 1$ we have:
\begin{align}
&D_{\alpha} (\Pi_t, Q_t) \\
=&  \frac{1- \int \left ( \frac{\pi_t(m)}{q_t(m)}\right ) ^{\alpha}q_t(m) dm}{\alpha(1-\alpha)} \\ 
=&  \frac{1- \int_{\Omega_1} \left ( \frac{\pi_t(m)}{q_t(m)}\right ) ^{\alpha} q_t(m) dm -\int_{\Omega_2} \left (\frac{\pi_t(m)}{q_t(m)}\right ) ^{\alpha}q_t(m) dm }{\alpha(1-\alpha)} \\ 
%- \frac{ \int_{\Omega_2} \left ( \frac{\pi_t(m)}{q_t(m)}\right ) ^{\alpha}q_t(m) dm}{\alpha(1-\alpha)} \\
=&  \frac{1- \int_{\Omega_1} \left ( r \right ) ^{\alpha}q_t(m) dm - \int_{\Omega_2} \left ( \frac{1 - \Pi_{t,1}}{1 - \Pi_{t,1}/r} \right ) ^{\alpha}q_t(m) dm}{\alpha(1-\alpha)} \\ 
%&-  \frac{ \int_{m_2 \geq m_1} \left ( \frac{1 - \Pi_{t,1}}{1 - \Pi_{t,1}/r} \right ) ^{\alpha}q_t(m) dm}{\alpha(1-\alpha)} \\ 
=&  \frac{1- Q_t(\Omega_1)\left ( r \right ) ^{\alpha} - Q_t(\Omega_2) \left ( \frac{1 - \Pi_{t,1}}{1 - \Pi_{t,1}/r} \right ) ^{\alpha}}{\alpha(1-\alpha)} \\ 
=&  \frac{1- \frac{\Pi_{t,1}}{r}\left ( r \right ) ^{\alpha} - (1 - \frac{\Pi_{t,1}}{r}) \left ( \frac{1 - \Pi_{t,1}}{1 - \Pi_{t,1}/r} \right ) ^{\alpha}}{\alpha(1-\alpha)} \\ 
\label{eq:max_d_alpha_large}
%=& \frac{1}{\alpha(1-\alpha)} \left ( 1 -  \Pi_{t,1} r^{-1+\alpha}- (1-\Pi_{t,1})^{\alpha} (1-\frac{\Pi_{t,1}}{r})^{1-\alpha} \right) \\
%=& \frac{1}{\alpha(\alpha-1 )} \left (  \Pi_{t,1} r^{-1+\alpha} + (1-\Pi_{t,1})^{\alpha} (1-\frac{\Pi_{t,1}}{r})^{1-\alpha} -1 \right)
\end{align}
%When $\alpha = 1$:
%\begin{align}
%   & D_{\alpha} (\Pi_t, Q_t) \\
%=&  \int \pi_t(m) \log \left ( \frac{\pi_t(m)}{q_t(m)} \right ) dm \\ 
%=& \int_{\Omega_1} \pi_t(m) \log \frac{\pi_t(m)}{q_t(m)} dm + \int_{\Omega_2} \pi_t(m) \log  \frac{\pi_t(m)}{q_t(m)} \ dm \\
%=& \int_{\Omega_1} \pi_t(m) \log(r) dm \\&+ \int_{\Omega_2} \pi_t(m) \log \frac{1 - \Pi_{t,1}}{1 - \Pi_{t,1}/r} dm \\
%=& \Pi_{t,1}\log(r) + (1-\Pi_{t,1})\log \frac{1 - \Pi_{t,1}}{1 - \Pi_{t,1}/r} 
%\end{align}
We will now upper bound the above expression.% Consider 2 cases
%\begin{itemize}
%    \item $\alpha =1$:   We have
%\begin{align}
%   & D_{\alpha} (\Pi_t, Q_t) \\
%&= \Pi_{t,1}\log(r) + (1-\Pi_{t,1})\log \frac{1 - \Pi_{t,1}}{1 - \Pi_{t,1}/r} \\
%&\leq \Pi_{t,1}\log(r) + (1-\Pi_{t,1})\log(r) \text{ because } r>1\\
%&\leq \log(r)
%\end{align}


%    \item $\alpha > 0, \alpha \neq 1$: 
The following inequality is true by simple calculations when $0< \alpha < 1$ or $\alpha > 1$: 
    \begin{align}
    \label{eq:upper_bound_error}
    \frac{(1-\Pi_{t,1})^{\alpha} (1-\frac{\Pi_{t,1}}{r})^{\alpha-1} }{\alpha(\alpha-1)} \leq \frac{(1-\Pi_{t,1}) r^{-1+\alpha}}{\alpha(\alpha -1 )}. 
\end{align}

Then we will have: 
    \begin{align}
  &D_{\alpha} (\Pi_t, Q_t)  \\
  = &\frac{\Pi_{t,1} r^{-1+\alpha} + (1-\Pi_{t,1})^{\alpha} (1-\frac{\Pi_{t,1}}{r})^{\alpha-1} -1}{\alpha(\alpha-1 )}  \\
 \leq & \frac{1}{\alpha(\alpha-1 )} \left (  \Pi_{t,1} r^{-1+\alpha} + (1-\Pi_{t,1}) r^{-1+\alpha} -1 \right) \\
 = &  \frac{1}{\alpha(\alpha-1 )} \left (   r^{-1+\alpha}  -1 \right).
\end{align}

%Now we will prove Eq.~\ref{eq:upper_bound_error}. 
%\begin{itemize}
%   \item When $0< \alpha < 1$: It is easy to check that
%    \begin{align}
%       \frac{ - (1-\Pi_{t,1})^{\alpha} (1-\frac{\Pi_{t,1}}{r})^{1-\alpha}}{\alpha(1-\alpha )}< \frac{- (1-\Pi_{t,1}) r^{\alpha-1}}{\alpha(1-\alpha )},
%    \end{align}
%    which is equivalent to:
%     \begin{align}
%         (1-\Pi_{t,1})^{\alpha} (1-\frac{\Pi_{t,1}}{r})^{1-\alpha} > (1-\Pi_{t,1}) r^{\alpha-1},
%    \end{align}
%    because 
%     \begin{align}
%       r^{1-\alpha} > \left( \frac{1-\Pi_{t,1}}{1-\frac{\Pi_{t,1}}{r}} \right)^{1- \alpha}.
%    \end{align}
%    
%    
%   \item When $\alpha > 1$:  We have
%    \begin{align}
%        (1-\Pi_{t,1})^{\alpha} (1-\frac{\Pi_{t,1}}{r})^{1-\alpha} < (1-\Pi_{t,1}) r^{\alpha-1}
%    \end{align}
%    because 
%     \begin{align}
%       \left( \frac{1-\Pi_{t,1}}{1-\frac{\Pi_{t,1}}{r}} \right)^{\alpha-1}  <  r^{\alpha-1}
%    \end{align}
%\end{itemize}
%Then we will have for all $0< \alpha, \alpha \neq 1$
%\begin{align}
%    D_{\alpha} (\Pi_t, Q_t)   
% \leq   \frac{1}{\alpha(\alpha-1 )} \left (   r^{-1+\alpha}  -1 \right). 
% \label{eq:epsilon_shape1} 
%\end{align}
%\end{itemize}
Therefore $D_{\alpha} (\Pi_t, Q_t)$ is upper bounded by:
\begin{align}
\label{eq:large_alpha}
%    \begin{cases}
    \frac{1- {r}^{\alpha-1}}{\alpha(1-\alpha)}, &\text{ if }  0 < \alpha <1  \text{ or } \alpha > 1\\
%    \log(r), &\text{ if } \alpha = 1 \\
 %      \frac{r^{\alpha-1}-1}{\alpha(\alpha-1)}, &\text{ if } \alpha > 1 \\
%    \end{cases}
\end{align}
Since %$\lim_{r \rightarrow 1} \log(r) = 0$ and
 $ \lim_{r \rightarrow 1} \frac{1- r^{-1+\alpha}}{\alpha(1-\alpha)} =0$, for any $\epsilon > 0$, there exists $r > 1$ such that
\begin{align}
D_{\alpha} (\Pi_t, Q_t) \leq \epsilon.
\end{align}
In Figure~\ref{fig:large_alpha}, we show the values of $\epsilon$ and $\alpha$  for a fixed $r$. 
\begin{figure}[ht]
    \centering
    \begin{subfigure}[t]{0.5\columnwidth}
    \centering
	\includegraphics[width=\columnwidth]{fig/large_alpha_r20.png}
	\caption{$D_{\alpha} (\Pi_t, Q_t)=\epsilon $ as a function of $\alpha$ when $r =2$}
    \end{subfigure}%
    ~ 
    \begin{subfigure}[t]{0.5\columnwidth}
    \centering
	\includegraphics[width=\columnwidth]{fig/large_alpha_r11.png}
	\caption{$D_{\alpha} (\Pi_t, Q_t) $ as a function of $\alpha$ when $r =1.1$}
\end{subfigure}
    \caption{\label{fig:large_alpha}$D_{\alpha} (\Pi_t, Q_t) =\epsilon$ as a function of $\alpha$ for the example in Theorem~\ref{thm:alpha_larger_than_0}}
\end{figure}
\end{proof}
\subsection{Proof of Lemma~\ref{lem:regret1}}
\begin{proof}
%	\begin{figure}[ht]
%		\centering
%		\includegraphics[width=\columnwidth]{fig/regret_epsilon1.png}
%		\caption{\label{fig:regret_epsilon1} Lower bound of regret per time step as a function of $\epsilon$ when $m_1 - m_2 = 0.1$ in the example in Theorem~\ref{thm:alpha_larger_than_0}}
%	\end{figure}
We will now lower bound the regret as a function of $\epsilon$. 

For any posterior $\Pi_t$, since the approximate algorithm sampling from $Q_t$ picks the optimal arm with probability at most $1/r$ then it picks arm $2$ with probability at least $1-1/r$. 
% The regret per time step can be lower bounded by $(m_1 - m_2)(1- 1/r)$. 

%From the condition of the prior: 

% \begin{align}
%     P(|M_1 - M_2| < \delta) < 1- \gamma
% \end{align}
% We choose $\delta = 0.5$ and $\gamma = 0.4$. Then 
% \begin{align}
%     P(|M_1 - M_2| \geq 0.5) > 0.4
% \end{align}
% Which implies either $P(M_2 - M_1 \geq 0.5) > 0.2$ or $P(M_1 - M_2 \geq 0.5) > 0.2$. WLOG assume:
% \begin{align}
%     P(M_1 - M_2 \geq 0.5) = 0.2
% \end{align}
Since we sample from $Q_t$ for $T'$ time steps, the lower bound of the average expected regret per time step is :
\begin{align}
    L =\frac{T'}{T} (m^*_1 - m^*_2)(1- 1/r) = c \Delta(1-1/r)
\end{align}
where $\Delta = m^*_1 - m^*_2$ and $c=\frac{T'}{T}$ is $\Theta(1)$

Since we have 
\begin{align}
    \epsilon &=  
    \begin{cases}
    \frac{1- r^{-1+\alpha}}{\alpha(1-\alpha)}, &\text{ if } \alpha \neq 1 \\
    log(r), &\text{ if } \alpha = 1
    \end{cases}
\end{align}
 
Then
\begin{align}
    \epsilon =
    \begin{cases}
    \frac{1- \left( \frac{1}{1-\frac{L}{c\Delta}}\right ) ^{-1+\alpha}}{\alpha(1-\alpha)}, &\text{ if } \alpha \neq 1 \\
    log\frac{1}{1-\frac{L}{c\Delta}}, &\text{ if } \alpha = 1
    \end{cases}
\end{align}
When $0<\alpha<1$, there is an upper bound on the error $\epsilon$ that is possible to get:
\begin{align}
    D_{\alpha} (\Pi_t, Q_t) &=\frac{1}{\alpha(\alpha-1 )} \left (   r^{-1+\alpha}  -1 \right) \\
    &\leq \frac{1}{\alpha(1-\alpha)},
\end{align}
so 
   \begin{align}
    L =
    \begin{cases}
    c\Delta(1- (1-\epsilon \alpha(1-\alpha))^{\frac{1}{1-\alpha}}), &\text{ if } \alpha > 1 \\
    c\Delta(1 - \frac{1}{e^{\epsilon}}), & \text{ if } \alpha = 1 \\
     c\Delta(1- (1-\epsilon  \alpha(1-\alpha))^{\frac{1}{1-\alpha}}),    & \parbox[t]{.3\columnwidth}{ if $0< \alpha < 1$ \\ and \\ $0 \leq \epsilon \leq \frac{1}{\alpha(1-\alpha)}$}, 
     \end{cases}
\end{align}
We plot the lower bound of the average regret per time step when $\Delta = 0.1$ as a function of $\epsilon$ in Fig~\ref{fig:regret_epsilon1}. 

\end{proof}
\subsection{The Average Regret per Time-step}
To understand how the constant average regret per time-step depends on $\epsilon$ and $\alpha$, we plot in Figure~\ref{fig:regret_epsilon1} the lower bound of the average regret per time-step as a function of $\epsilon$ in the following setting of the example constructed in the proof of Theorem~\ref{thm:alpha_larger_than_0}. The algorithm samples from $Q_t$ at $T/2$ time-steps and $\Delta = 0.1$. In this case the average regret per time step is upper bounded by $\Delta/2 = 0.05$. The formula and proof are detailed in Lemma~\ref{lem:regret1} in Appendix~\ref{sec:proof_alpha_larger_than_0}. 
\begin{figure}[ht]
	\centering
	\includegraphics[width=\columnwidth, height = 5cm, keepaspectratio]{fig/regret_epsilon1.png}
	\caption{\label{fig:regret_epsilon1} Lower bound of regret per time-step as a function of $\epsilon$ when $m^*_1 - m^*_2 = 0.1$ and we sample from the approximation for $T/2$ time-steps in the example construted in the proof of Theorem~\ref{thm:alpha_larger_than_0}. When $\alpha$ is around $1$, the lower bound converges quickly as $\epsilon$ increases.}
\end{figure}
When $\alpha$ is around $1$, the lower bound, and therefore the average regret per time-step, converges the fastest to $\Delta/2$ as $\epsilon$ increases. When $\alpha$ is very large or close to $0$, the lower bound grows slowly as $\epsilon$ increases.%When $\alpha$ is close to $0$, the average regret grows slowly as $\epsilon$ increases. 
%.

==> proof_thm_alpha_smaller_than_1.tex <==
\section{Proof of Theorem \ref{thm:alpha_less_than_1_example}}
\label{sec:proof_alpha_less_than_1}
Let $\Pi_{t,i}$ denote $\Pi_t(\Omega_i)$. We construct the pdf of $Q_t$'s as follows: 
\begin{align}
\label{eq:Q_t_construction_alpha_less_than_1}
q_t(m) = 
\begin{cases}
\frac{1}{\Pi_{t,2}} \pi_t(m), \text{ if } m_2 > m_1 \\
0, \text{ otherwise}. 
\end{cases}
\end{align}

We will prove the theorem by the following steps:
\begin{itemize}
    \item In Lemma~\ref{lem:valid_distribution_alpha_smaller_than_1} we show that $Q_t$'s are valid distributions. 
    \item In Lemma~\ref{lem:small_divergence_alpha_less_than_1} we show that there exists a bad prior such that the $\alpha$-divergence between $Q_t$ and $\Pi_t$ can be arbitrarily small for $\alpha > 0$.
    \item In Lemma~\ref{lem:regret_alpha_less_than_1} we show that $Q_t$ has linear regret, and calculate the constant average regret per time-step.
\end{itemize}

\begin{lemma}
\label{lem:valid_distribution_alpha_smaller_than_1}
If $\int \pi_t(m) dm = 1$ then the density function $q_t$ defined in Eq.~\ref{eq:Q_t_construction_alpha_less_than_1} satisfies:
\begin{align}
\int q_t(m) dm = 1. 
\end{align}
\end{lemma}


\begin{lemma}
\label{lem:small_divergence_alpha_less_than_1}
When $\alpha < 1$, 

For any $ \epsilon > 0$, there exists  a prior $\Pi_0$ where $M_1-M_2$ and $M_2$ are independent such that for any posterior $\Pi_t$ and approximation $Q_t$ constructed in Eq.~\ref{eq:Q_t_construction_alpha_less_than_1},  $D_{\alpha} (\Pi_t, Q_t) < \epsilon$. 

For any  prior $\Pi_0$ where $M_1-M_2$ and $M_2$ are independent,  there exists $\epsilon > 0 $ such that for any posterior $\Pi_t$ and approximation $Q_t$ constructed in Eq.~\ref{eq:Q_t_construction_alpha_less_than_1},  $D_{\alpha} (\Pi_t, Q_t) < \epsilon$. 
\end{lemma}

\begin{lemma}
\label{lem:regret_alpha_less_than_1}
The expected regret of the policy that constructs $Q_t$'s as in Eq.~\ref{eq:Q_t_construction_alpha_less_than_1} is linear and the average regret per time-step is $\Delta = m^*_1-m^*_2$. 
%   \begin{align}
%    L = 
%    \begin{cases}
%    \Delta(1 - (1-\epsilon \alpha (1-\alpha))^{1/\alpha}), &\parbox[t]{.3\columnwidth}{ if $0< \alpha < 1$ \\ and \\ $0 \leq \epsilon \leq \frac{1}{\alpha(1-\alpha)}$},  \\ 
%    \Delta(1 - \frac{1}{e^{\epsilon}}), &\text{ if } \alpha = 0 \\
%    \Delta(1 - (1-\epsilon \alpha (1-\alpha))^{1/\alpha}),& \text{ if } \alpha <0. 
%    \end{cases}
%\end{align}
\end{lemma}
\subsection{Proof of Lemma~\ref{lem:valid_distribution_alpha_smaller_than_1}}
\begin{proof}
Assume that $\int \pi_t(m) dm = 1$, we will show that $\int q_t(m) dm = 1$: 
\begin{align}
  &\int q_t(m) dm \\ 
  &= \int_{\Omega_1}  q_t(m) dm + \int_{\Omega_2}  q_t(m) dm \\ 
  &= 0 + \int_{\Omega_2}   \frac{1}{ \Pi_{t,2}} \pi_t(m) dm \\
  &= \frac{1}{ \Pi_{t,2}} \int_{\Omega_2}    \pi_t(m) dm \\
  &= 1
\end{align}
\end{proof}
\subsection{Proof of Lemma~\ref{lem:small_divergence_alpha_less_than_1}}
\begin{proof} 
We will show that $M_1 - M_2$ and $H_{t-1}$ are independent. Since the algorithm always chooses arm $2$, $M_1$ and $H_{t-1}$ are independent given $M_2$, which implies $M_1-M_2$ and $H_{t-1}$ are independent given $M_2$. Since $M_1 - M_2$ and $M_2$ are also independent, we have:
\begin{align}
&\mathbb{P}(M_1-M_2 |M_2, H_{t-1})  \\ =  &\mathbb{P}(M_1-M_2 |M_2) \\ = &\mathbb{P}(M_1-M_2). 
\end{align}
Then 
\begin{align}
&\mathbb{P}(M_1-M_2 | H_{t-1}) \\
=  &\int \mathbb{P}(M_1-M_2 |M_2= m_2, H_{t-1})  \mathbb{P}(M_2=m_2 |H_{t-1}) dm_2 \\
=  &\int  \mathbb{P}(M_1-M_2|M_2 = m_2) \mathbb{P}(M_2=m_2 |H_{t-1}) dm_2 \\
=  &\mathbb{P}(M_1 - M_2) \int  \mathbb{P}(M_2=m_2 |H_{t-1}) dm_2 \\
=  &\mathbb{P}(M_1 - M_2) . 
\end{align}
Then at all time $t$:
\begin{align}
\Pi_{t,2}& =\mathbb{P}(M_1-M_2 < 0 |H_{t-1}) = \mathbb{P}(M_1< M_2) 
\end{align}
For simplicity let
\begin{align}
	z:=\mathbb{P}(M_1< M_2)
\end{align}
We will show that  $D(\Pi_t, Q_t)$ is small. First we calculate the $\alpha$-divergence between $\Pi_t$ and $Q_t$ constructed in Eq~\ref{eq:Q_t_construction_alpha_less_than_1}. 

When $\alpha <1, \alpha \neq 0$: 
\begin{align}
&D_{\alpha} (\Pi_t, Q_t)  \\
=&  \frac{1- \int \left ( \frac{q_t(m)}{\pi_t(m)}\right ) ^{1-\alpha} \pi_t(m) dm}{\alpha(1-\alpha)} \\ 
=&  \frac{1 - \int_{\Omega_1} \left ( \frac{q_t(m)}{\pi_t(m)}\right ) ^{1-\alpha} \pi_t(m) dm -\int_{\Omega_2} \left ( \frac{q_t(m)}{\pi_t(m)}\right ) ^{1-\alpha} \pi_t(m) dm }{\alpha(1-\alpha)} \\ 
 % & - \frac{\int_{\Omega_2} \left ( \frac{q_t(m)}{\pi_t(m)}\right ) ^{1-\alpha} \pi_t(m) dm}{\alpha(1-\alpha)} \\
=&  \frac{1- 0  - \int_{\Omega_2} \left ( \frac{1}{\Pi_{t,2}}\right ) ^{1-\alpha} \pi_t(m) dm}{\alpha(1-\alpha)} \text{ since } \alpha < 1 \\
=&  \frac{1- \left (\frac{1}{\Pi_{t,2}} \right ) ^{1-\alpha}\int_{\Omega_2}   \pi_t(m) dm}{\alpha(1-\alpha)} \\
=&  \frac{1- \left (\frac{1}{\Pi_{t,2}} \right ) ^{1-\alpha} \Pi_{t,2}}{\alpha(1-\alpha)} \\
=&  \frac{1 - (\Pi_{t,2}) ^{\alpha}}{\alpha(1-\alpha)} \\ 
=& \frac{1-z^{\alpha}}{\alpha(1-\alpha)}
\end{align}
%When $\alpha = 0$: 
%\begin{align}
%    &D_{\alpha} (\Pi_t, Q_t) \\ =& \int q_t(m) \log  \frac{q_t(m)}{\pi_t(m)} dm \\
%    =& \int_{\Omega_1} q_t(m) \log  \frac{q_t(m)}{\pi_t(m)} dm  \\ &+ \int_{\Omega_2} q_t(m) \log \frac{q_t(m)}{\pi_t(m)} dm  \\
%    =& \int_{\Omega_1} 0 \log(0)dm + \int_{\Omega_2} q_t(m) \log \frac{1}{\Pi_{t,2}}dm \\
%    = &0 + 1 \log  \frac{1}{\Pi_{t,2}} = \log  \frac{1}{\Pi_{t,2}}= \log  \frac{1}{z}
%\end{align}
Note that if we don't have the condition on the prior such that picking arm $2$ does not help to learn which arm is the better one, $\Pi_{t,2}$ may converge to $0$, making $D_{\alpha} (\Pi_t, Q_t)$ goes to $\infty$ when $\alpha \leq 0 $. But since $\Pi_{t,2}=z$, we will now show that for any $\alpha <1$, for any $\epsilon >0$, there exists $z (0 <z <1)$ such that  
\begin{align}
    D_{\alpha} (\Pi_t, Q_t) < \epsilon
\end{align}
%Consider the 2 cases
%\begin{itemize}
    %\item 
    When $\alpha <1, \alpha \neq 0$: Since
    \begin{align}
   \lim_{z \rightarrow 1}  \frac{1-z^{\alpha}}{\alpha(1-\alpha)} =0
   \end{align}
   Then for any $\epsilon > 0 $ there exists $z, 0 < z< 1$ such that $D_{\alpha}(\Pi_t, Q_t) < \epsilon$.
   For any $z< 1 $ there exists $\epsilon > 0$ such that $D_{\alpha}(\Pi_t, Q_t) < \epsilon$
   
%   \item  When $\alpha = 0$: 
%    \begin{align}
%    D_{\alpha} (\Pi_t, Q_t) &=   \log  \frac{1}{z}
%\end{align}
%Since $\lim_{z \rightarrow 1} \log(1/z) = 0 $, for any $\epsilon > 0 $ there exists $z, 0 < z< 1$ such that $D_0(\Pi_t, Q_t) < \epsilon$. For any $z< 1 $ there exists $\epsilon > 0$ such that $D_{\alpha}(\Pi_t, Q_t) < \epsilon$
%\end{itemize}
\end{proof}
\subsection{Proof of Lemma~\ref{lem:regret_alpha_less_than_1}}
\begin{proof}
According to the approximate distribution, arm $2$ is chosen with probability $1$ at all times. 
Clearly this approximate distribution has linear regret.
Therefore $\Delta=m^*_1 - m^*_2$ is the average regret per time-step.
% When $z=1$, the approximation is exact but still has linear regret because the prior is very bad.
% For each $M = m$ where $m_1 > m_2$, since the algorithm always pick $a_2$ the cumulative at time $T$ is $(m_1 - m_2)T$. For each $M=m$ where $m_2 > m_1$ the regret is $0$
% We made further assumptions for the prior stated in Eq.~\ref{eq:prior_property2}. From the condition of the prior: 
% \begin{align}
%     P(M_1 - M_2 >0.4) = 1- r
% \end{align}
% The Bayesian regret is the expectation over the prior of $M$
% \begin{align}
%     \mathbb{R}(T) &= \mathbb{E}_M (m_1 - m_2)T \\
%     &= T\int_{m_1 > m_2} (m_1 - m_2) \pi_0(m_1,m_2) dm \\
%     &\geq T\int_{m_1 > m_2 + 0.4} 0.4 \pi_0(m_1,m_2) dm \\
%     &\geq 0.4(1-r)T
% \end{align}
% which depends on the prior
%Since $Q_t$ always pick the sub-optimal arm, let $L = \Delta(1-z)$ denote the lower bound of the average regret per time step where $\Delta = m^*_1 - m^*_2$. Then $z = 1 - \frac{L}{\Delta}$. 
%Since 
%\begin{align}
%    \epsilon = 
%    \begin{cases}
%    \frac{1-z^\alpha}{\alpha(1-\alpha)}, &\text{ if } \alpha \neq 0 \\
%     \log\frac{1}{r}, &\text{ if } \alpha = 0
%    \end{cases}
%\end{align}
%we have
%\begin{align}
%    \epsilon = 
%    \begin{cases}
%    \frac{1-(1 - \frac{L}{\Delta})^\alpha}{\alpha(1-\alpha)},  &\text{ if } \alpha \neq 0 \\
%    \log\frac{1}{1 - \frac{L}{\Delta}}, \text{ if } \alpha = 0
%    \end{cases}
%\end{align}
%When $0<\alpha<1$, there is an upper bound on the error $\epsilon$ that is possible to get:
%\begin{align}
%    D_{\alpha} (\Pi_t, Q_t) &=\frac{1}{\alpha(1-\alpha)} \left ( 1-  z^{\alpha}  \right) \\
%    &\leq \frac{1}{\alpha(1-\alpha)}
%\end{align}
%so 
%   \begin{align}
%    L = 
%    \begin{cases}
%    \Delta(1 - (1-\epsilon \alpha (1-\alpha))^{1/\alpha}), &\parbox[t]{.3\columnwidth}{ if $0< \alpha < 1$ \\ and \\ $0 \leq \epsilon \leq \frac{1}{\alpha(1-\alpha)}$},  \\ 
%    \Delta(1 - \frac{1}{e^{\epsilon}}), &\text{ if } \alpha = 0 \\
%    \Delta(1 - (1-\epsilon \alpha (1-\alpha))^{1/\alpha}),& \text{ if } \alpha <0. 
%    \end{cases}
%\end{align}
\end{proof}


==> proof_uniform.tex <==
\section{Proof of Lemma~\ref{thm:uniform_sublinear_regret}}
\label{sec:proof_uniform}
%From Lemma~\ref{lem:convert_distribution}, $D_{\alpha}(\Pi_t, Q_t) <\epsilon $ implies $D_{\alpha} (\overline{\Pi_t}, \overline{Q_t}) < \epsilon$, therefore in order to prove Theorem~\ref{thm:uniform_sublinear_regret} we prove the following lemma with the stronger condition: 
%\begin{lemma}
%	\label{lem:uniform_sublinear_regret}
%	For any number of arms $ k$, for any prior  $\Pi_0$, for any error threshold $\epsilon > 0$, the following algorithm that at every time step $t$:
%	\begin{itemize}
%		\item with probability $1-\frac{1}{{t}}$, samples from an approximate posterior $Q_t$ such that $D_{\alpha} (\overline{\Pi_t}, \overline{Q_t}) < \epsilon$, and
%		\item with probability $\frac{1}{{t}}$ , samples an arm uniformly at random.
%	\end{itemize}
%	has $o(T)$ regret. 
%\end{lemma}


Without loss of generalization, let arm $1$ be the best arm. From Lemma~\ref{lem:posterior_concentration}, since $\sum_t^{\infty} p_t = \infty$, every arm is chosen infinitely often and therefore with probability $1$:
\begin{align}
\lim_{t \rightarrow \infty} \mathbb{P}(A^*=1|H_{t-1}) = 1, 
\end{align}
which means that the posterior probability that arm $1$ is the best arm converges to $1$. 

We will prove the lemma by proving the following steps: 
\begin{itemize}
    \item In Lemma~\ref{lem:approximation_convergence} we show that if the probability that the posterior chooses the best arm tends to $1$, then the probability that the approximation chooses the best arm also tends to $1$
    \item In Lemma~\ref{lem:sublinear_regret} and Lemma~\ref{lem:sublinear_regret2} we show that if the probability that the approximation chooses the best arm also tends to $1$, then it has sub-linear regret
\end{itemize}

We can now show that when the posterior concentrates and the $\alpha$-divergence is smaller than a threshold, the approximate distribution also concentrates. 
\begin{lemma}
\label{lem:approximation_convergence}
Let $\alpha \leq 0$ and  arm $1$ be the true best arm. Let $\Omega_i =\{m | m_i = max (m_1, ..., m_k)\}$ be the region where arm $i$ is the best arm. If the posterior probability that arm $1$ is the best arm converges to $1$: 
\begin{align}
    \lim_{t \rightarrow \infty}  \Pi_{t,1} = 1 
\end{align}
and 
\begin{align}
D_{\alpha} (P,Q) < \epsilon,
\end{align}
then the sequence $\{Q_{t,1}\}_t$ where $ Q_{t,1} = \int_{\Omega_1} q_t(m) dm$ converges and 
\begin{align}
     \lim_{t \rightarrow \infty} Q_{t,1} = 1\;.
\end{align}
\end{lemma}


Next we show that if the approximate distribution concentrates, then the probability that it chooses the wrong arm decreases  as $T$ goes to infinity. 
\begin{lemma}
\label{lem:sublinear_regret}
If 
\begin{align}
     \lim_{t \rightarrow \infty} Q_{t,1} = 1 
\end{align}
then 
\begin{align}
   \lim_{T \rightarrow \infty} \frac{\sum_{t=1}^T (1- Q_{t,1}) }{T}= 0\;.
\end{align}
\end{lemma}
Since $\lim_{t \rightarrow \infty}  \Pi_{t,1} = 1$, then $\lim_{T \rightarrow \infty} \frac{\sum_{t=1}^T (1- Q_{t,1}) }{T}= 0$ with proability $1$. We will now show that the expected regret is sub-linear:
\begin{lemma}
	\label{lem:sublinear_regret2}
	 Let $p_t= o(1)$ be such that $\sum_t^\infty p_t = \infty$. For any number of arms $ k$, any prior  $\Pi_0$ and any error threshold $\epsilon > 0$, the following algorithm has $o(T)$ regret: at every time-step $t$,
	 \begin{itemize}
	 	\item with probability $1-p_t$, sample from an approximate posterior $Q_t$ such that $\lim_{T \rightarrow \infty} \frac{\sum_{t=1}^T (1- Q_{t,1}) }{T}= 0 $ with probability $1$, and
	 	\item with probability $p_t$, sample an arm uniformly at random.
	 \end{itemize}
\end{lemma}
\subsection{Proof of Lemma~\ref{lem:approximation_convergence}}
\begin{proof}
% First we will show that 
% \begin{align}
% \label{eq:alpha_divergence_0}
% f(p, q) = q\log\frac{q}{p}
% \end{align}
% and 
% \begin{align}
% \label{eq:alpha_divergence_neq_0}
% f(p, q) = \frac{p^{\alpha}q^{1-\alpha}} {\alpha ( \alpha-1)}
% \end{align}
% are convex in order to apply Lemma~\ref{lem:convert_distribution}.
% The Hessian matrix of Eq.~\ref{eq:alpha_divergence_0}
% is:
% \begin{align}
%     \begin{bmatrix}
%      \frac{q}{p^2} & -\frac{1}{p} \\
%     -\frac{1}{p} & \frac{1}{q}
%     \end{bmatrix}
% \end{align}
% with eigenvalues:
% \begin{align}
%     \lambda_1 &= 0 \\
%     \lambda_2 &= \frac{p^2+q^2}{p^2q}
% \end{align}
% Since both the eigenvalues are non-negative, the matrix is positive semi-definite, so Eq~\ref{eq:alpha_divergence_0} is convex.
% The Hessian matrix of Eq.~\ref{eq:alpha_divergence_neq_0}
% is 
% \begin{align}
%     \begin{bmatrix}
%     p^{\alpha-2}q^{1-\alpha} & -p^{\alpha-1}q^{-\alpha} \\
%     -p^{\alpha-1}q^{-\alpha} & p^{\alpha}q^{-\alpha-1}
%     \end{bmatrix}
% \end{align}
% with eigenvalues
% \begin{align}
%     \lambda_1 &= 0 \\
%     \lambda_2 &= p^{\alpha -2} q^{-\alpha-1} (p^2+q^2)
% \end{align}
% Since both the eigenvalues are non-negative, the matrix is positive semi-definite, so Eq~\ref{eq:alpha_divergence_neq_0} is convex. 

Let 
$Q_{t,i} = \int_{\Omega_i} q_t(m) dm$ and $\Pi_{t,i} = \int_{\Omega_i} \pi_t(m) dm$.
Then 
\begin{align}
    \lim_{t \rightarrow \infty} \Pi_{t,1} = 1
\end{align} and we want to show that $\{Q_{t,1}\}_t$ converges and 
\begin{align}
    \lim_{t \rightarrow \infty} Q_{t,1} = 1.
\end{align} 
%We consider the 2 cases: 
%\begin{itemize}
%	\item When $\alpha = 0$:
%	\begin{align}
%	D_{\alpha}(\overline{\Pi}_t,\overline{Q}_t) = \sum_{i=1}^k Q_{t,i} \log \frac{Q_{t,i}}{\Pi_{t,i}}  
%	\end{align}
%	Since $D_{\alpha}(\overline{\Pi_t},\overline{Q_t}) < \epsilon$ and $\lim \Pi_{t,1} =1$ we want to show that $\limsup Q_{t,1} =1$. 
%	By contradiction, assume that: 
%	\begin{align}
%	\limsup  Q_{t,1} = c < 1. 
%	\end{align}
%	Then there exists a sub-sequence of $\{Q_{t,1}\}_t$, denoting $Q_{t_1, 1}, Q_{t_2, 1}, ..., Q_{t_n, 1},..$ such that
%	\begin{align}
%	\label{eq:lim_subsequence1}
%	\lim_{n \rightarrow \infty} Q_{t_n, 1} = c.
%	\end{align}
%	
%	which implies 
%		\begin{align}
%		0< 1- c = \lim_{n \rightarrow \infty} \sum_{i=2}^k  Q_{t_n, i} \leq  \sum_{i=2}^k \limsup_{n \rightarrow \infty} Q_{t_n, i}.
%		\end{align}
%	Therefore there exists $j \in [2,k]$ such that: 
%	   \begin{align}
% \limsup_{n \rightarrow \infty} Q_{t_n, j}= d > 0
%	   \end{align}
%	Then there exists a sub-sequence of $\{Q_{t_n,j}\}_n$, denoting $Q_{t_{n_1}, j}, Q_{t_{n_2}, j}, ..., Q_{t_{n_m}, j},..$ such that
%	\begin{align}
%	\lim_{m \rightarrow \infty} Q_{t_{n_m}, j} = d.
%	\end{align}
%	Then we have:
%	\begin{align}
%	\epsilon = &\lim_{m \rightarrow \infty} D_{\alpha}(\overline{\Pi}_{t_{n_m}}, \overline{Q}_{t_{n_m}}) \\
%	\geq & \lim_{m \rightarrow \infty}  Q_{t_{n_m},1} \log \frac{Q_{t_{n_m},1}}{\Pi_{t_{n_m},1}}  +\lim_{m \rightarrow \infty}  Q_{t_{n_m},j} \log \frac{Q_{t_{n_m},j}}{\Pi_{t_{n_m},j}} \\
%	= &  c\log\frac{c}{1} + d\log \frac{d}{0} \\
%	= & \infty \text{ since } d > 0, 
%	\end{align}
%	which is a contradiction. Therefore $c = 1$. 
%	
%	Similarly we will show that: 
%	\begin{align}
%	\liminf Q_{t,1} = 1.
%	\end{align}
%		By contradiction, assume that: 
%		\begin{align}
%		\liminf  Q_{t,1} = c' < 1. 
%		\end{align}
%		Then there exists a sub-sequence of $\{Q_{t,1}\}_t$, denoting $Q_{t_1, 1}, Q_{t_2, 1}, ..., Q_{t_{n'}, 1},..$ such that
%		\begin{align}
%		\lim_{n \rightarrow \infty} Q_{t_{n'}, 1} = c' .
%		\end{align}
%		Using the same argument following Eq.~\ref{eq:lim_subsequence1} we will have $c'=1$. 
%	Since $\liminf Q_{t,1} = \limsup Q_{t,1} = 1$, we have that $Q_{t,1}$ converges and
%	\begin{align}
%	\lim Q_{t,1} = 1.
%	\end{align}
%	\item 
When $\alpha < 0$: 
	
	\begin{align}
	&D_{\alpha}(\overline{\Pi}_t,\overline{Q}_t) 
	= \frac{ \sum_{i=1}^k \Pi_{t,i}^{\alpha} Q_{t,i}^{1-\alpha} - 1} {\alpha(\alpha-1)} 
	\end{align}
	Since $D_{\alpha}(\overline{\Pi_t},\overline{Q_t})  < \epsilon$ and $\lim \Pi_{t,1} =1$ we want to show  that $\limsup Q_{t,1} =1$. 
		By contradiction, assume that: 
		\begin{align}
		\limsup  Q_{t,1} = c < 1. 
		\end{align}
		Then there exists a sub-sequence of $\{Q_{t,1}\}_t$, denoting $Q_{t_1, 1}, Q_{t_2, 1}, ..., Q_{t_n, 1},..$ such that
		\begin{align}
		\label{eq:lim_subsequence2}
		\lim_{n \rightarrow \infty} Q_{t_n, 1} = c.
		\end{align}
		
		which implies 
		\begin{align}
		0< 1- c = \lim_{n \rightarrow \infty} \sum_{i=2}^k  Q_{t_n, i} \leq  \sum_{i=2}^k \limsup_{n \rightarrow \infty} Q_{t_n, i}.
		\end{align}
		Therefore there exists $j \in [2,k]$ such that: 
		\begin{align}
		\limsup_{n \rightarrow \infty} Q_{t_n, j}= d > 0
		\end{align}
		Then there exists a sub-sequence of $\{Q_{t_n,j}\}_n$, denoting $Q_{t_{n_1}, j}, Q_{t_{n_2}, j}, ..., Q_{t_{n_m}, j},..$ such that
		\begin{align}
		\lim_{m \rightarrow \infty} Q_{t_{n_m}, j} = d.
		\end{align}
	Then we have: 
	\begin{align}
	\epsilon = &\lim_{m \rightarrow \infty} D_{\alpha}(\overline{\Pi}_{t_{n_m}}, \overline{Q}_{t_{n_m}}) \\
	\geq & \lim_{m \rightarrow \infty}  \frac{\Pi_{t_{n_m},1}^{\alpha} Q_{t_{n_m},1}^{1-\alpha} + \Pi_{t_{n_m},j}^{\alpha} Q_{t_{n_m},j}^{1-\alpha}  - 1} {\alpha(\alpha-1)}  \\
	= &  \frac{1^{\alpha} c^{1-\alpha} + \frac{d^{1-\alpha}}{(0)^{-\alpha}}  - 1} {\alpha(\alpha-1)} \\
	= & \infty, \text{ since } d > 0 \text{ and } \alpha < 0,
	\end{align}
	which is a contradiction. Therefore $c = 1$. 
	
		Similarly we will show that: 
		\begin{align}
		\liminf Q_{t,1} = 1.
		\end{align}
		By contradiction, assume that: 
		\begin{align}
		\liminf  Q_{t,1} = c' < 1. 
		\end{align}
		Then there exists a sub-sequence of $\{Q_{t,1}\}_t$, denoting $Q_{t_1, 1}, Q_{t_2, 1}, ..., Q_{t_{n'}, 1},..$ such that
		\begin{align}
		\lim_{n \rightarrow \infty} Q_{t_{n'}, 1} = c' .
		\end{align}
		Using the same argument following Eq.~\ref{eq:lim_subsequence2} we will have $c'=1$. 
	Since $\liminf Q_{t,1} = \limsup Q_{t,1} = 1$, we have that $\{Q_{t,1}\}_t$ converges and
	\begin{align}
	\lim Q_{t,1} = 1.
	\end{align}
%\end{itemize}
%First we will show that if we are sampling with error $\epsilon$ with respect to the distribution of the means $M$, then we are also choosing the best arm from an approximating distribution with error at most $\epsilon$. First we use Lemma~\ref{lem:Jensen} to lower bound the $\alpha$-divergence in term of $Q_{t,1}$ and $\Pi_{t,1}$:
%\begin{itemize}
%\item When $\alpha = 0$:
%\begin{align}
%    &D_{\alpha}(\Pi_t,Q_t) \\
%    =& \int q_t(m) \log \frac{q_t(m)}{\pi_t(m)} dm \\
%    =& \int_{\Omega_1} q_t(m) \log \frac{q_t(m)}{\pi_t(m)} dm + \int_{\overline{\Omega_1}} q_t(m) \log \frac{q_t(m)}{\pi_t(m)} dm \\
%    \geq&|\Omega_1| \frac{1}{|\Omega_1|} \int_{\Omega_1} q_t(m) dm \log \frac{\frac{1}{|\Omega_1|}\int_{\Omega_1} q_t(m) dm}{\frac{1}{|\Omega_1|}\int_{\Omega_1} \pi_t(m) dm}  \\& + |\overline{\Omega_1}| \frac{1}{|\overline{\Omega_1}|}\int_{\overline{\Omega_1}} q_t(m) dm \log \frac{\frac{1}{|\overline{\Omega_1}|}\int_{\overline{\Omega_1}} q_t(m) dm}{\frac{1}{|\overline{\Omega_1}|}\int_{\overline{\Omega_1}} \pi_t(m) dm} \\
%    &\text{ by applying Lemma~\ref{lem:Jensen}} \\
%    =&  Q_{t,1} \log \frac{Q_{t,1}}{\Pi_{t,1}}  +(1-Q_{t,1}) \log \frac{(1-Q_{t,1})}{(1-\Pi_{t,1})}. 
%\end{align}
%Since $D_{\alpha}(P,Q) < \epsilon$ and $\lim \Pi_{t,1} =1$ we want to show that $\limsup Q_{t,1} =1$. 
%By contradiction, assume that: 
%\begin{align}
%    \limsup  Q_{t,1} = c < 1. 
%\end{align}
%Then there exists a sub-sequence of $Q_{t,1}$, denoting $Q_{t_1, 1}, Q_{t_2, 1}, ..., Q_{t_n, 1},..$ such that
%\begin{align}
%    \lim_{n \rightarrow \infty} Q_{t_n, 1} = c
%\end{align}
%Then we have:
%\begin{align}
%    &\lim_{n \rightarrow \infty} D_{\alpha}(\Pi_{t_n,1}, Q_{t_n,1}) \\
%    = & \lim_{n \rightarrow \infty}  Q_{t_n,1} \log \frac{Q_{t_n,1}}{\Pi_{t_n,1}}  +(1-Q_{t_n,1}) \log \frac{(1-Q_{t_n,1})}{(1-\Pi_{t_n,1})} \\
%    = &  c\log\frac{c}{1} + (1-c)\log \frac{1-c}{0} \\
%    = & \infty \text{ since } 1-c > 0, 
%\end{align}
%which is a contradiction. Therefore $c = 1$. 
%Similarly we can show that: 
%\begin{align}
%    \liminf Q_{t,1} = 1.
%\end{align}
%Since $\liminf Q_{t,1} = \limsup Q_{t,1} = 1$, we have that $Q_{t,1}$ converges and
%\begin{align}
%    \lim Q_{t,1} = 1.
%\end{align}
%\item When $\alpha < 0$: 
%
%\begin{align}
%    &D_{\alpha}(P_t,Q_t) \\
%    =&  \int \frac{p(x)^{\alpha}q(x)^{1-\alpha} - 1 }{-\alpha(1-\alpha)} dx\\
%    =& \frac{-1}{\alpha(\alpha -1) } +  \int_{\Omega_1} \frac{p(x)^{\alpha}q(x)^{1-\alpha} }{\alpha(\alpha-1)} dx  \\ &+  \int_{\overline{\Omega_1}} \frac{p(x)^{\alpha}q(x)^{1-\alpha} }{\alpha(\alpha-1)} dx \\
%    \geq& \frac{-1}{\alpha(\alpha -1) }  +  |\Omega_1| \frac{ (\frac{\Pi_{t,1}}{|\Omega_1|})^{\alpha} (\frac{Q_{t,1}}{|\Omega_1|})^{1-\alpha}} {\alpha(\alpha-1)} \\
%    +& |\overline{\Omega_1}| \frac{(\frac{1-\Pi_{t,1}}{|\overline{\Omega_1}|})^{\alpha} (\frac{1-Q_{t,1}}{|\overline{\Omega_1}|})^{1-\alpha}} {\alpha(\alpha-1)} \\
%        &\text{ by applying Lemma~\ref{lem:Jensen}} \\
%    =& \frac{\Pi_{t,1}^{\alpha} Q_{t,1}^{1-\alpha} + (1-\Pi_{t,1})^{\alpha} (1-Q_{t,1})^{1-\alpha} - 1} {\alpha(\alpha-1)} 
%\end{align}
%Since $D_{\alpha}(P,Q) < \epsilon$ and $\lim \Pi_{t,1} =1$ we want to show that $\liminf Q_{t,1} =1$. Since $D_{\alpha}(P,Q) < \epsilon$ and $\lim \Pi_{t,1} =1$ we want to show that $\limsup Q_{t,1} =1$. 
%By contradiction, assume that: 
%\begin{align}
%    \limsup  Q_{t,1} = c < 1. 
%\end{align}
%Then there exists a sub-sequence of $Q_{t,1}$, denoting $Q_{t_1, 1}, Q_{t_2, 1}, ..., Q_{t_n, 1},..$ such that
%\begin{align}
%    \lim_{n \rightarrow \infty} Q_{t_n, 1} = c. 
%\end{align}
%Then we have: 
%\begin{align}
%    &\lim_{n \rightarrow \infty} D_{\alpha}(\Pi_{t_n,1}, Q_{t_n,1}) \\
%    = & \lim_{n \rightarrow \infty}  \frac{\Pi_{t_n,1}^{\alpha} Q_{t_n,1}^{1-\alpha} + (1-\Pi_{t_n,1})^{\alpha} (1-Q_{t_n,1})^{1-\alpha} - 1} {\alpha(\alpha-1)}  \\
%    = &  \frac{1^{\alpha} c^{1-\alpha} + \frac{(1-c)^{1-\alpha}}{(0)^{-\alpha}}  - 1} {\alpha(\alpha-1)} \\
%    = & \infty, \text{ since } 1-c > 0 \text{ and } \alpha < 0,
%\end{align}
%which is a contradiction. Therefore $c = 1$. 
%Similarly we can show that: 
%\begin{align}
%    \liminf Q_{t,1} = 1.
%\end{align}
%Since $\liminf Q_{t,1} = \limsup Q_{t,1} = 1$, we have that $Q_{t,1}$ converges and
%\begin{align}
%    \lim Q_{t,1} = 1.
%\end{align}
%\end{itemize}
\end{proof}
\subsection{Proof for Lemma~\ref{lem:sublinear_regret}}
For simplicity let $x_t$ denote $1- Q_{t,1}$. We want to show that if a sequence $\{x_t\}$ satisfies $x_t \geq 0 ~\forall t$ and: 
\begin{align}
     \lim_{t \rightarrow \infty} x_t = 0,
\end{align}
then 
\begin{align}
  \lim_{T \rightarrow \infty} S_T = 0,
\end{align}
where 
\begin{align}
S_T= \frac{\sum_{t=1}^T x_t }{T}. 
\end{align}

Since $ \lim_{t \rightarrow \infty} x_t = 0$ and $x_t \geq 0~\forall t$, for any $\epsilon > 0$ there exists $T_0$ such that for all $t > T_0$:
\begin{align}
    x_t < \frac{\epsilon}{2}
\end{align}
Then for all $T > T_0$: 
\begin{align}
    S_T & = \frac{x_1 + ... + x_{T_0}}{T} + \frac{x_{T_0+1} + ... + x_T}{T} \\
    & \leq \frac{x_1 + ... + x_{T_0}}{T} + \frac{\frac{\epsilon}{2} T}{T} \\
    & \leq \frac{x_1 + ... + x_{T_0}}{T} + \frac{\epsilon}{2}
\end{align}
Choose $T_1$ large enough such that $ \frac{x_1 + ... + x_{T_0}}{T_1} < \frac{\epsilon}{2}$. Let $T_2 = \max(T_0, T_1)$. Then for all $T > T_2$: 
\begin{align}
    S_T = \frac{x_1 + ... + x_{T_0}}{T} + \frac{\epsilon}{2} < \frac{\epsilon}{2} + \frac{\epsilon}{2} = \epsilon
\end{align}
Therefore for any $\epsilon > 0$, there exists $T_2$ such that for all $T > T_2$, $S_T < \epsilon$. Since $S_T \geq 0~\forall T$, we have: 
\begin{align}
    \lim_{T \rightarrow \infty} S_T = 0
\end{align}
\subsection{Proof of Lemma~\ref{lem:sublinear_regret2}}
Without loss of generalization, let arm $1$ be the true best arm. Let $\Delta = m^*_1- \min(m^*_1, ..., m^*_k)$ be the gap between the highest mean $m^*_1$ and the lowest mean of the arms. 

Since $p_t = o(1)$, $\sum_{t=1}^T p_t $ is $o(T)$. Therefore the regret from the uniform sampling steps is $o(T)$. 

Since $1-Q_{t,1}$ is the probability of choosing a sub-optimal arm by sampling from $Q_t$, the regret of sampling from  $Q_t$ is upper bounded by:
\begin{align}
\mathbb{E}\sum_{t=1}^T \Delta (1-Q_{t,1})
\end{align}
Since $   \lim_{T \rightarrow \infty} \frac{\sum_{t=1}^T (1- Q_{t,1}) }{T}= 0 $ with probability $1$, we have
\begin{align}
\lim_{T \rightarrow \infty} \frac{\sum_{t=1}^T \Delta (1- Q_{t,1}) }{T}= 0,
\end{align}
with probability $1$. Therefore the expected regret of sampling from $Q_t$ is sub-linear.

Since both the expected regrets of the uniform sampling steps and of sampling from $Q_t$ is sub-linear, the total expected regret is sub-linear. 

==> simulation_diagram.tex <==
\begin{figure}[ht]
	\centering
% \begin{subfigure}[t]{0.4\textwidth}
% 	\centering
% 	\begin{tikzpicture}
% 	[align=center,node distance=1.2cm]
% 	\node (pi0) [dist] {$\Pi_0$};
% 	\node (A1) [action, right of = pi0] {$A_1$};
% 	\node (pi1) [dist, below of= pi0] {$\Pi_1$};
% 	\node (A2) [action, right of = pi1] {$A_2$};
% 	\node (pi2) [dist, below of =pi1] {$\Pi_2$};
% 	\node (A3) [action, right of = pi2] {$A_3$};
% 	\node (Y1) [action, right of = A1] {$Y_1$};
% 	\node (Y2) [action, right of = A2] {$Y_2$};
% 	\node (Y3) [action, right of = A3] {$Y_3$};
% 	
% 	\draw [thick, ->] (pi0) -- (A1);
% 	\draw [thick, ->] (pi1) -- (A2);
% 	\draw [thick, ->]  (pi2) -- (A3);
% 	\draw [thick, ->] (A1) -- (Y1);
% 	\draw [thick, ->] (A2) -- (Y2);
% 	\draw [thick, ->]  (A3) -- (Y3);
% 	\draw [thick, ->]  (pi0) -- (pi1);
% 	\draw [thick, ->]  (pi1) -- (pi2);
% 	\draw [thick, ->]  (Y1) -- (pi1);
% 	\draw [thick, ->] (Y2) -- (pi2);
% 	\end{tikzpicture}
% 	\caption{\label{fig:exact_TS_diagram} Exact Thompson sampling.}
% \end{subfigure}
% \hfill
 \begin{subfigure}[t]{0.44\textwidth}
 	\centering
 	\begin{tikzpicture}
 	[align=center,node distance=1.2cm]
 	\node (pi0) [dist] {$\Pi_0$};
 	\node (q0) [approx_dist, right of = pi0] {$Q_0$};
 	\node (A1) [action, right of = q0] {$A_1$};
 	\node (pi1) [dist, below of= pi0] {$\Pi_1$};
 	\node (q1) [approx_dist, right of = pi1] {$Q_1$};
 	\node (A2) [action, right of = q1] {$A_2$};
 	\node (pi2) [dist, below of =pi1] {$\Pi_2$};
 	\node (q2) [approx_dist, right of = pi2] {$Q_2$};
 	\node (A3) [action, right of = q2] {$A_3$};
 	\node (Y1) [action, right of = A1] {$Y_1$};
 	\node (Y2) [action, right of = A2] {$Y_2$};
 	\node (Y3) [action, right of = A3] {$Y_3$};
 	
 	\draw [thick, ->] (pi0) -- (q0);
 	\draw [thick, ->] (pi1) -- (q1);
 	\draw [thick, ->]  (pi2) -- (q2);
 	\draw [thick, ->] (q0) -- (A1);
 	\draw [thick, ->] (q1) -- (A2);
 	\draw [thick, ->]  (q2) -- (A3);
 	
 	\draw [thick, ->]  (pi0) -- (pi1);
 	\draw [thick, ->]  (pi1) -- (pi2);
 	\draw [thick, ->] (A1) -- (Y1);
 	\draw [thick, ->] (A2) -- (Y2);
 	\draw [thick, ->]  (A3) -- (Y3);
 	\draw [thick, ->]  (Y1) -- (pi1);
 	\draw [thick, ->] (Y2) -- (pi2);
 	\end{tikzpicture}
 	\caption{\label{fig:approx_TS_diagram} Thompson sampling with approximation $Q_t$}
 \end{subfigure}
 		\hfill
 		\begin{subfigure}[t]{0.52\textwidth}
 			\begin{tikzpicture}
 			[align=center,node distance=1.1cm]
 		
 				\node (pi0) [dist] {$\Pi_0$};
 				\node (q0) [approx_dist, right of = pi0] {$Q_0$};
 				\node (A1) [action, right of = q0] {$A_1$};
 				\node (pi1) [dist, below of= pi0] {$\Pi_1$};
 				\node (q1) [approx_dist, right of = pi1] {$Q_1$};
 				\node (A2) [action, right of = q1] {$A_2$};
 				\node (pi2) [dist, below of =pi1] {$\Pi_2$};
 				\node (q2) [approx_dist, right of = pi2] {$Q_2$};
 				\node (A3) [action, right of = q2] {$A_3$};
 				\node (Y1) [action, right of = A1] {$Y_1$};
 				\node (Y2) [action, right of = A2] {$Y_2$};
 				\node (Y3) [action, right of = A3] {$Y_3$};
 				
 				\draw [thick, ->] (pi0) -- (q0);
 				\draw [thick, ->] (pi1) -- (q1);
 				\draw [thick, ->]  (pi2) -- (q2);
 				\draw [thick, ->] (q0) -- (A1);
 				\draw [thick, ->] (q1) -- (A2);
 				\draw [thick, ->]  (q2) -- (A3);
 				
 				\draw [thick, ->]  (pi0) -- (pi1);
 				\draw [thick, ->]  (pi1) -- (pi2);
 				\draw [thick, ->] (A1) -- (Y1);
 				\draw [thick, ->] (A2) -- (Y2);
 				\draw [thick, ->]  (A3) -- (Y3);
 				
 				
 				\node (Ap1) [action, left of = pi0] {$A'_1$};
 				\node (Ap2) [action, left of = pi1] {$A'_2$};
 				\node (Ap3) [action, left of = pi2] {$A'_3$};
 				\node (Yp1) [action, left of = Ap1] {$Y'_1$};
 				\node (Yp2) [action, left of = Ap2] {$Y'_2$};
 				\node (Yp3) [action, left of = Ap3] {$Y'_3$};
 				
 				\draw [thick, ->] (pi0) -- (Ap1);
 				\draw [thick, ->] (pi1) -- (Ap2);
 				\draw [thick, ->]  (pi2) -- (Ap3);
 				\draw [thick, ->] (Ap1) -- (Yp1);
 				\draw [thick, ->] (Ap2) -- (Yp2);
 				\draw [thick, ->]  (Ap3) -- (Yp3);
 				\draw [thick, ->]  (Yp1) -- (pi1);
 				\draw [thick, ->] (Yp2) -- (pi2);
 				
 			\end{tikzpicture}
 			\caption{\label{motivating_example_simulation_diagram} Thompson sampling with approximation $Q_t$ calculated from the posterior updated by exact Thompson sampling.}
 		\end{subfigure}
% 		\hfill
% 		\begin{subfigure}[t]{0.15\textwidth}
% 			\begin{tikzpicture}
% 			[align=center,node distance=1cm]
% 			\node (pi0) [dist] {$\Pi_0$};
% 			\node (q0) [approx_dist, right of = pi0] {$Z_0$};
% 			\node (A1) [action, right of = q0] {$A_1$};
% 			\node (pi1) [dist, below of= pi0] {$\Pi_1$};
% 			\node (q1) [approx_dist, right of = pi1] {$Z_1$};
% 			\node (A2) [action, right of = q1] {$A_2$};
% 			\node (pi2) [dist, below of =pi1] {$\Pi_2$};
% 			\node (q2) [approx_dist, right of = pi2] {$Z_2$};
% 			\node (A3) [action, right of = q2] {$A_3$};
% 			\draw [thick, ->] (pi0) -- (q0);
% 			\draw [thick, ->] (pi1) -- (q1);
% 			\draw [thick, ->]  (pi2) -- (q2);
% 			\draw [thick, ->] (q0) -- (A1);
% 			\draw [thick, ->] (q1) -- (A2);
% 			\draw [thick, ->]  (q2) -- (A3);
% 			
% 			\draw [thick, ->]  (pi0) -- (pi1);
% 			\draw [thick, ->]  (pi1) -- (pi2);
% 			\draw [thick, ->]  (A1) -- (pi1);
% 			\draw [thick, ->] (A2) -- (pi2);
% 			\end{tikzpicture}
% 			\caption{Thompson sampling with approximation $Z_t$.}
% 		\end{subfigure}
% 		\hfill
% 		\begin{subfigure}[t]{0.2\textwidth}
% 			\begin{tikzpicture}
% 			[align=center,node distance=1cm]
% 			
% 			\node (pi0) [dist] {$\Pi_0$};
% 			\node (q0) [approx_dist, right of = pi0] {$Z_0$};
% 			\node (A1) [action, right of = q0] {$A_1$};
% 			\node (pi1) [dist, below of= pi0] {$\Pi_1$};
% 			\node (q1) [approx_dist, right of = pi1] {$Z_1$};
% 			\node (A2) [action, right of = q1] {$A_2$};
% 			\node (pi2) [dist, below of =pi1] {$\Pi_2$};
% 			\node (q2) [approx_dist, right of = pi2] {$Z_2$};
% 			\node (A3) [action, right of = q2] {$A_3$};
% 			\draw [thick, ->] (pi0) -- (q0);
% 			\draw [thick, ->] (pi1) -- (q1);
% 			\draw [thick, ->]  (pi2) -- (q2);
% 			\draw [thick, ->] (q0) -- (A1);
% 			\draw [thick, ->] (q1) -- (A2);
% 			\draw [thick, ->]  (q2) -- (A3);
% 			
% 			\draw [thick, ->]  (pi0) -- (pi1);
% 			\draw [thick, ->]  (pi1) -- (pi2);
% 			
% 			\node (Aprime1) [action,left of = pi0] {$A'_1$};
% 			\node (Aprime2) [action, left  of = pi1] {$A'_2$};
% 			\node (Aprime3) [action, left  of = pi2] {$A'_3$};
% 			\draw [thick, ->] (pi0) -- (Aprime1);
% 			\draw [thick, ->] (pi1) -- (Aprime2);
% 			\draw [thick, ->]  (pi2) -- (Aprime3);
% 			\draw [thick, ->]  (Aprime1) -- (pi1);
% 			\draw [thick, ->] (Aprime2) -- (pi2);
% 			\end{tikzpicture}
% 			\caption{Thompson sampling with approximation $Z_t$ calculated from the posterior updated by exact Thompson sampling.}
% 		\end{subfigure}
 			\caption{\label{fig:motivating_example_simulation_diagram}}
\end{figure}

